Using human and robot synthetic data for training smart hand tools

The future of work does not require a choice between human and robot. Aside from explicit human-robot collaboration, robotics can play an increasingly important role in helping train workers as well as the tools they may use, especially in complex tasks that may be difficult to automate or effectively roboticize. This paper introduces a form of smart tool for use by human workers and shows how training the tool for task recognition, one of the key requirements, can be accomplished. Machine learning (ML) with purely human-based data can be extremely laborious and time-consuming. First, we show how data synthetically-generated by a robot can be leveraged in the ML training process. Later, we demonstrate how fine-tuning ML models for individual physical tasks and workers can significantly scale up the benefits of using ML to provide this feedback. Experimental results show the effectiveness and scalability of our approach, as we test data size versus accuracy. Smart hand tools of the type introduced here can provide insights and real-time analytics on efficient and safe tool usage and operation, thereby enhancing human participation and skill in a wide range of work environments. Using robotic platforms to help train smart tools will be essential, particularly given the diverse types of applications for which smart hand tools are envisioned for human use.

==> paper_chapters/3-system-architecture-updated.tex <==
\section{System Architecture} \label{sec:SysArch}
\subsection{Smart Tool Module (STM)} \label{sec:SmartHandTool}

The apparatus developed in this work serves as a platform for demonstrating real-world applications of the smart tool concept. The intent is to formulate a set of best practices applicable to the development of smart tools for various work application areas. The particular sensor module used in this work is composed of eleven different sensors including a 9-axis inertial measurement unit (IMU), a microphone, and an ammeter. During the operation of the hand tool, the sensors generate data that is recorded and analyzed by both RaspberryPi microcomputer and Arduino microcontroller. Additionally, a small OLED screen is embedded in the smart tool module (STM) for communicating with the operator. A custom-made encasing protects the sensors and data collection hardware from the environment. The IMU, microphone, OLED ccreen, and 5-way switch are mounted to the STM and placed in a 3D-printed box encased in aluminum.% The setup can be replicated with low-effort soldering and manufacturing skills.

A rotary power tool (RPT), specifically the Model 4300AC by Dremel (Racine, WI, USA), was chosen as the platform for testing the smart tool concept. A typical RPT is shown in Figure \ref{fig:teaser}. This hand-held power tool has an electrical AC motor directly coupled to a drive-shaft that can be manually adjusted by a user to rotate at a desired speed (5,000 to 35,000 revolutions per minute, or rpm). Different tool bits can be attached to the drive-shaft to change the tool function. A RPT is not intended to be used in applications that will require high levels of force from the operator; instead, the operator guides the tool to control its interaction with the workpiece material. There are a wide range of attachments that enable a RPT to be used for many different purposes such as polishing, grinding, cutting, and routing. The versatility of the RPT and the variety of manual control actions required by the human user were key reasons for selecting it for this preliminary study in smart tool development.

\subsection{Yaskawa Robot}\label{sec:YaskawaRobot}

\figSysArch

\figClamping

The Yaskawa SDA10D robot is an industrial robot that is equipped with two robotic arms that operate independently. The robot features dual 7-axis arms, which enables it to exhibit human-like flexibility when performing a variety of movements. Moreover, its programming environment is highly adaptable, as it provides the ability to modify not only position values but also speed and acceleration. The robot can be controlled by manipulating each of its joints individually, or alternatively, by regulating the XYZ position of the end effector.

To accomplish the tasks set out in Section~\ref{sec:Experimental-Results} and produce synthetic data, a programmable automatic machine was needed, in this case the Yaskawa SDA10D robot, was selected due to its ability to execute movements similar to those of a human using a hand tool. Prior to programming the movement patterns and constructing the tool fastening system to the end effector of the robot arm, the variables involved in routing, sanding, engraving, and cutting processes that a human would undertake were examined. 

Human execution of these tasks is not consistent, as it is a stochastic process due to the compliance of the human arm that reacts to the resistance of the material being machined, specifically for this experiment an anisotropic material such as wood. Furthermore, variables such as speed, trajectory, working depth, working and travel angles generated by humans are subject to variation. 

To imitate these conditions and owing to the fact that robotic movements are uniform and devoid of variability, a robotic arm-tool fastening system that provides some freedom of movement via adjustable threaded clamps were developed. Additionally, a piece of rubber is situated between the robot and the tool to replicate the compliance resulting from human operation, as shown in Figure~\ref{fig:FasteningSystem}. This system enables us to replicate the variation in trajectory, compliance, and work and travel angles. To introduce variability in the working depth and speed, programming of the robot was undertaken.

The programming of movement patterns for each activity was executed using cartesian control based on the coordinates of the robotic arm's end effector. Specifically, XYZ coordinates were determined to simulate human-like movements of routing, sanding, engraving, and cutting with a dremel tool. The working depth was programmed based on the maximum and minimum values observed during human performance using an RPT, with the depth value being adjusted with each tool pass. A trapezoidal velocity profile was selected for the cartesian control programming. By combining these parameters allows for a better dispersion of data that is comparable to that produced by a human. 

All of the programming was carried out using Robot Operating System (version Noetic Ninjemys) in C++. After we identified pattern of movements, we encoded them into 6-DOF vector for each of the tasks. 

It is noteworthy that the same RPT, sensor suite, and experimental setup used for human data collection was mounted on the robotic arm for data collection purposes. This ensures experimental consistency.


\subsection{Data Collection}\label{sec:DataCollection}
Our software stack comprises three main components: data collection, data cleaning, and model building. We describe all three in some detail as follows.

The data collection process is facilitated by an Arduino microcontroller that communicates with the sensor rig on the RPT. The Arduino is responsible for collecting dataframes in the form of CSV files containing the sensor readings. The data collection process was carried out using two methods: the first involved human subjects performing the tasks, while the second utilized the Yaskawa Robot (as described in Section~\ref{sec:YaskawaRobot}.

Once data was collected, we performed data cleaning to remove outliers. The human-collected data was found to be relatively "dirtier" than the robot-collected data, and we removed about 30\% of the human data after outlier removal. In contrast, the robot-collected data was cleaner as the robot was programmed to perform the tasks consistently for every run. We removed only about 10\% of robot-collected data after the outlier removal process.

Consenting volunteers were instructed on how to use the instrumented RPT in the four activities: cutting, engraving, routing, and sanding, with the bits shown in Figure \ref{fig:toolbits}. A high-level verbal description with minimal instructions were given for each activity as follows:

\figToolBits

\textbf{Cutting.} A 1.5 inch wood cutting wheel is installed on the tool and a 0.5 inch diameter round wooden dowel rod is secured to a workbench. The user is asked to slice approximately 1/4 inch discs over the span of a given time period.

\textbf{Engraving.} An engraving bit is installed on the rotary tool and a piece of standard `2-by-4' lumber measuring 12 inches in length was secured to a workbench. Each user was asked to engrave numbers from zero through nine continuously over a given time period.

\textbf{Routing.} A straight routing bit is installed on the rotary tool and a piece of standard `2-by-4' lumber measuring 12 inches in length was secured to a workbench. Each user routes approximately one-eighth inch deep grooves across the width of the wood over the designated time period.

\textbf{Sanding.} A sanding drum is installed on the rotary tool. The subject creates a one half inch \emph{chamfer} on every edge of the `2-by-4' lumber over a designated time period.
    
The participants were given instructions on how to set-up the different tool bits. Some pointers on how to use the tool for a given task were provided, but users were given freedom to achieve each task based on their own comfort with the tool, experience, and unique style. This approach was taken to allow for variability in how each person operated the tool and completed the task.
    
Data collection was conducted for about a one and a half month period. A total of seven participants (five graduate students and two faculty) used the instrumented RPT to work on wooden samples. Each sample run was set for three minutes. A total of 204 sample runs or 612 minutes of data was collected.  After each test, the `2-by-4' wood samples were collected and organized for future analysis. In addition, each run was video recorded for future research work using images and raw sound.

Data was collected from a total of seven different participants over the span of 1.5 months. Each participant performed nine runs of each of the 4 tasks. The nine runs were broken down into 3 runs of training data, 3 runs of validation data, and 3 runs of testing data. A total of 204 sample runs or 612 minutes of data were collected.

Two participants were used for Out-of-Distribution (OoD) testing. The purpose of OoD testing is to analyze the model's performance on unseen data generated from completely new subjects that were not used in training. This step is important because it examines the effectiveness of the model at generalizing to different users. Additionally, one OoD subject's data was collected with the same tool and in the same environment as the train subjects. The other OoD subject's data was collected with a duplicate tool and in a different environment in order to further test generalization.
 
After collecting data from each subject performing the four different activities, three CSV files were concatenated into three different data frames containing the raw data for train, validate, and test data. Then, these raw data frames were preprocessed to produce offline training data for the ML models. Data pre-processing involved breaking down the data into 10 second frames with 50\% overlap. The frame size was selected through an iterative process which
resulted in 10 seconds producing the best results, while the 50\% overlap was chosen to feed the model more data. Ten statistical features (minimum, maximum, kurtosis, standard error of the mean, standard deviation, variance, sample skewness, median absolute deviation, and sum) where extracted from each sensor measurement (9 axis IMU, microphone, current sensor) for a total of 110 features. Subsequently, the data was normalized to values from 0 to 1.
